A fast and slightly robust covariance estimator

Let $\mathcal{Z} = \{Z_1, \dots, Z_n\} \stackrel{\mathrm{i.i.d.}}{\sim} P \subset \mathbb{R}^d$ from a distribution $P$ with mean zero and covariance $\Sigma$. Given a dataset $\mathcal{X}$ such that $d_{\mathrm{ham}}(\mathcal{X}, \mathcal{Z}) \leq \varepsilon n$, we are interested in finding an efficient estimator $\widehat{\Sigma}$ that achieves $\mathrm{err}(\widehat{\Sigma}, \Sigma) := \|\Sigma^{-\frac{1}{2}}\widehat{\Sigma}\Sigma^{-\frac{1}{2}} - I\| _{\mathrm{op}} \leq 1/2$. We focus on the low contamination regime $\varepsilon = o(1/\sqrt{d}$). In this regime, prior work required either $\Omega(d^{3/2})$ samples or runtime that is exponential in $d$. We present an algorithm that, for subgaussian data, has near-linear sample complexity $n = \widetilde{\Omega}(d)$ and runtime $O((n+d)^{\omega + \frac{1}{2}})$, where $\omega$ is the matrix multiplication exponent. We also show that this algorithm works for heavy-tailed data with near-linear sample complexity, but in a smaller regime of $\varepsilon$. Concurrent to our work, Diakonikolas et al. [2024] give Sum-of-Squares estimators that achieve similar sample complexity but with large polynomial runtime.

==> sections/alg-analysis.tex <==
\section{$\alg$ analysis}
% \subsection{Overview}
% \subsubsection{Definitions}
% % \begin{definition}
% %   (good direction) A direction $v \in \S^{d-1}$ is $\alpha$-good for $M \succeq 0 \in \R^{d \times d}$ if
% %   \begin{align*}
% %     v^T \Sigma^{-1/2}M \Sigma^{-1/2}v \leq 1+\alpha.
% %   \end{align*}
% % \end{definition}
% \begin{definition}
%   (bad direction) A direction $v \in \S^{d-1}$ is $\beta$-bad for $M \succeq 0 \in \R^{d \times d}$ if
%   \begin{align*}
%     v^T \Sigma^{-1/2}M \Sigma^{-1/2}v \geq 1+\beta.
%   \end{align*}
% \end{definition}

% \subsubsection{Proof sketch}
% \begin{itemize}
%   \item ($\Sigma_R$ not too big) ALG does not terminate while there exist $1$-bad directions for $\Sigma_R$.
%         \begin{itemize}
%           \item enough bad points have high inner products with each other that $\Sigma_S$ will have a large eigenvalue
%                 if there exist bad directions (Lemmas~\ref{lem:tail-lb} and \ref{lemma:negative-correlation-bound})
%         \end{itemize}
%   \item ($\Sigma_R$ not too small) ALG terminates with $\absv{G \setminus R} = O(\eps n)$.
%         \begin{itemize}
%           \item randomized filter will not remove more good points than bad points in expectation assuming $v^T \Sigma_{S \cap B} v \geq v^T \Sigma_{S \cap G} v$ (Chapter 3 in textbook)
%           \item maximum eigenvalue of $\Sigma_{S \cap G}$ is small
%                 \begin{itemize}
%                   \item if $S$ contains $o(n)$ good points, then maximum eigenvalue of $\Sigma_{S \cap G}$ will be small due to resilience (Lemma~\ref{lem:heavy-op-norm-resilience})
%                   \item assuming all points in $R$ have bounded $\Sigma_R$ norm, only $o(n)$ good points will have high inner product with other good points
%                         \begin{itemize}
%                           \item (concentration) for $n$ i.i.d. samples from $P$, most covariance-normalized inner products with respect to the empirical covariance will be $O(\sqrt{d})$; specifically, at most $o(n)$ points will have inner product $\omega(\sqrt{d})$ with another point (Lemma~\ref{lemma:inner-product-concentration})
%                           \item (subtractive contamination) after removing any $\eps$ fraction of points from the above i.i.d. dataset, it will still be the case that at most $o(n)$ points will have covariance-normalized inner product $\omega(\sqrt{d})$ with another point with respect to the new empirical covariance (Lemma~\ref{lemma:inner-prod-subtractive})
%                           \item (strong contamination) after adding $\eps n$ arbitrary chosen ``bad" points to the above dataset, it will still be the case that at most $o(n)$ non-bad points will have covariance-normalized inner product $\omega(\sqrt{d})$ with another point with respect to the new empirical covariance, so long as these ``bad'' points all have bounded Mahalanobis norm with respect to this empirical covariance (some version of Section 5.3.1)
%                         \end{itemize}
%                   \item all points in $R$ will have bounded $\Sigma_R$ norm after we apply the norm filter before initializing $S$ in ALG, and the norm filter will not filter any non-bad points (TODO: prove this; should be easy)\footnote{for heavy-tailed data we might get a better sample complexity when actually filtering some non-bad points; may have to adjust the algorithm to handle this case}
%                 \end{itemize}
%         \end{itemize}
%   \item (runtime - not critical)\footnote{worst case we can get an upper bound of $n$ iterations} ALG terminates in $\txt{polylog}(n)$ iterations.
%         \begin{itemize}
%           \item TODO: use analysis from Section 3.3 of textbook (will have to modify filtering step accordingly)
%         \end{itemize}
% \end{itemize}

\input{sections/main-result.tex}

\input{sections/single-iteration-analysis.tex}

\input{sections/randomized-filter-analysis.tex}

==> sections/conclusion.tex <==
\section{Conclusion and future work}
We presented the algorithm $\alg$ for robust covariance estimation in relative
spectral norm in the low-contamination regime
$\eps = o(1/\sqrt{d})$.
Moreover, we showed that $\alg$ requires only nearly-linear sample complexity
in the both the hypercontractive subgaussian and heavy-tailed regimes.
$\alg$ achieves this by iteratively identifying pairs of points that have
large inner-product with respect to the empirical covariance and
then filtering those points if they have large norm in a contaminated direction.
While Sum-of-Squares algorithms can solve already this problem in
$\poly(n, d)$ time, this runtime may still be too large in practice.
On the other hand, $\alg$ has a runtime of only $O(...)$, which is a bit more
than the time it take to multiply an $n \times d$ matrix by its transpose.

The major limitation of $\alg$ is that it only works in the
$\eps = o(1/\sqrt{d})$ regime.
This is because contaminated points only need inner products of
order $1/\eps$ to make the contaminated covariance have high error.
Thus, when $1/\eps = o(\sqrt{d})$, we cannot distinguish these contaminated
inner products from the inner products of good points which are
on the order of $\pm \ti{O}(\sqrt{d})$.
One potential way to extend our analysis to larger regimes of $\eps$ might be
to compare cliques of points with pairwise large inner product rather than
merely pairs of points.
At the cost of additional runtime, this might pick out directions where
many contaminated points conspire induce high error in the contaminated covariance.

Another limitation of $\alg$ is in the runtime.
In particular, we currently argue that in the worst case, only one point
is removed per iteration of the outer while-loop of $\alg$,
leading to $O(\eps n)$ total iterations.
We believe that with either a tighter analysis of the randomized filter or
a slight modification to $\alg$, one can show that only $O(\log n)$ iterations
are required with high probability, yielding a runtim of $O(...)$.

We leave addressing these limitations to future work.

==> sections/goodness-kmom-old.tex <==
\subsection{Heavy-tailed}
\begin{definition}
  A mean zero isotropic random vector $X$ has $k$th moment bounded by $m_k$ if
  for all $v \in \R^d$,
  \begin{align*}
    \E[|X \cdot v|^k]^{1/k} \leq m_k\norm{v}.
  \end{align*}
\end{definition}

% \begin{lemma}
%   Suppose $Y_1, \dots Y_n$ are scalar-valued, independent, mean $0$,
%   and $k$th moment bounded by $C$, then
%   \begin{align*}
%     \P\left(\frac{1}{n}\sum_{i=1}^n Y_i \geq \alpha \right)
%     &\leq 2\left(\sqrt{\frac{ek}{2}}\cdot \frac{C}{\alpha\sqrt{n}}\right)^{k}.
%   \end{align*}
% \end{lemma}
% \begin{proof}
%   \begin{align*}
%     \P\left(\frac{1}{n}\sum_{i=1}^n Y_i \geq \alpha \right)
%     &\leq \P\left((\sum_{i=1}^n Y_i)^k \geq (n\alpha)^k \right) \\
%     &\leq \frac{1}{(n\alpha)^k}\E[(\sum_{i=1}^n Y_i)^k].
%   \end{align*}
%   To proceed, we have by the multinomial theorem that
%   \begin{align*}
%     \E[(\sum_{i=1}^n Y_i)^k]
%     &= \sum_{1 \leq i_1, \dots, i_k \leq n} \E[Y_{i_1} \dots Y_{i_k}].
%   \end{align*}
%   Notice that for any choice of $i_1, \dots, i_k$ such that any specific value
%   occurs exactly once, the expectation is $0$ by the mean 0 assumption.
%   For other choices of $i_1, \dots, i_k$, the expectation is bounded by
%   $C^k$ by independence and Jensen's inequality.
%   Thus, we count the number of ways to choose $i_1, \dots, i_k$ such that
%   all values never appear exactly once.
%   Following Tao,
%   let $N_r$ be the number of ways to assign $i_1, \dots, i_k$ such that
%   exactly $k/2-r$ values appear.
%   Then, $N_r \leq (en)^{k/2 - r}(k/2)^{k/2+r}$.
%   Thus the total number of assignments is bounded by
%   \begin{align*}
%     \sum_{r=0}^{k/2} N_r
%     \leq \left(\frac{ekn}{2}\right)^{k/2}
%       \sum_{r=0}^{k/2} \left(\frac{k}{2en}\right)^r
%     \leq \left(\frac{ekn}{2}\right)^{k/2} \left(\frac{1}{1-\frac{k}{2en}}\right)
%     \leq 2 \left(\frac{ekn}{2}\right)^{k/2}.
%   \end{align*}
%   Thus,
%   \begin{align*}
%     \P\left(\frac{1}{n}\sum_{i=1}^n Y_i \geq \alpha \right)
%     &\leq 2\left(\sqrt{\frac{ek}{2}}\cdot \frac{C}{\alpha\sqrt{n}}\right)^{k}.
%   \end{align*}
% \end{proof}

\begin{lemma}[Concentration of empirical covariance]\label{lem:bdd-emp-cov-conc}
  For $\delta > 0$, if the $Z_i$ have $k$th moment bounded by $m_k$,
  then with probability at least $1-\delta$,
  \begin{align*}
    \norm{\hat{\Sigma} - I}
    = O\left(m_k^2 \delta^{-2/k} \max\{\sqrt{k d}n^{-1/2}, k d n^{2/k-1}\}\right).
  \end{align*}
\end{lemma}
\begin{proof}
  We first have that
  \begin{align*}
    \E[\norm{Z}^k]
    &= \E[(\norm{Z}^2)^{k/2}]
    = \E\left[\left(d \cdot \frac{1}{d}\sum_{j=1}^d (Z \cdot e_j)^2\right)^{k/2}\right]
    \leq d^{k/2} \E\left[\frac{1}{d}\sum_{j=1}^d |Z \cdot e_j|^k\right]
    \leq m_k^k d^{k/2}.
  \end{align*}
  By Markov's inequality,
  \begin{align*}
    \P(\big\|\hat{\Sigma} - I\big\| \geq \alpha)
    &= \P\left(\Big\|\sum_{i=1}^n (Z_iZ_i^T - I)\Big\| \geq \alpha n\right)
    \leq (\alpha n)^{-k/2} \E\left[\Big\|\sum_{i=1}^n (Z_iZ_i^T - I)\Big\|^{k/2}\right].
  \end{align*}
  Using \cite[Theorem A.1]{Tropp} we have that
  \begin{align*}
    \E\left[\Big\|\sum_{i=1}^n (Z_iZ_i^T - I)\Big\|^{k/2}\right]^{2/k}
    &\leq \sqrt{\frac{ek}{2}}\Big\|\left(n \E[(ZZ^T - I)^2]\right)^{1/2}\Big\|
      + ek\E[\max_i \norm{Z_iZ_i^T - I}^{k/2}]^{2/k}.
    % &\leq \sqrt{\frac{ekn}{2}}\Big\|\left(\E[\norm{X}^2XX^T] - I\right)^{1/2}\Big\|
    %   + ekn^{2/k}\E[\norm{XX^T - I}^{k/2}]^{2/k} \\
    % &\leq \sqrt{\frac{ekn}{2}}\Big\|\E[\norm{X}^2XX^T]\Big\|^{1/2}
    %   + ekn^{2/k}\E[|\norm{X}^2 - 1|^{k/2}]^{2/k} \\
    % &\leq \sqrt{\frac{ekn}{2}} (m_k^2 \sqrt{d})
    %   + ekn^{2/k}(1 + \E[\norm{X}^k]^{2/k}) \\
    % &\leq \sqrt{\frac{ekn d}{2}}m_k^2 + ekn^{2/k}(1+m_k^2 d) \\
    % &\leq Cm_k^2 \max\{\sqrt{k n d}, kn^{2/k} d\}.
  \end{align*}
  For the first term, we have that
  \begin{align*}
    \norm{\E[(ZZ^T - I)^2]^{1/2}}
    &= \norm{\E[\norm{Z}^2 ZZ^T - I]^{1/2}}.
  \end{align*}
  Note that
  \begin{align*}
    v^T\E[\norm{Z}^2 ZZ^T - I]v
    = \E[\norm{Z}^2 (Z \cdot v)^2] - 1
    \geq \E[(Z \cdot v)^4] - 1
    \geq \E[(Z \cdot v)^2]^2 - 1
    \geq 0,
  \end{align*}
  implying that $\E[\norm{Z}^2 ZZ^T] - I \succeq 0$, which further implies
  \begin{align*}
    \norm{\E[\norm{Z}^2 ZZ^T - I]^{1/2}}
    = \norm{\E[\norm{Z}^2 ZZ^T - I]}^{1/2}
    \leq \norm{\E[\norm{Z}^2 ZZ^T]}^{1/2}.
  \end{align*}
  Now for any $v \in \S^{d-1}$,
  \begin{align*}
    v^T\E[\norm{Z}^2 ZZ^T] v
    &= \E[\norm{Z}^2 (Z \cdot v)^2]
    \leq \E[|Z \cdot v|^k]^{2/k} \E[\norm{Z}^{2(1-2/k)^{-1}}]^{1-2/k}
    \leq m_k^2 \E[\norm{Z}^{\frac{2k}{k-2}}]^{\frac{k-2}{k}}.
  \end{align*}
  Because $k \geq 4$, we have that $\frac{2}{k-2} \leq 1$, and so
  \begin{align*}
    \E[\norm{Z}^{\frac{2k}{k-2}}]^{\frac{k-2}{k}}
    \leq \E[\norm{Z}^k]^{2/k}
    \leq m_k^2 d.
  \end{align*}
  This all implies
  \begin{align*}
    \norm{\E[(ZZ^T - I)^2]^{1/2}}
    \leq (m_k^{4} d)^{1/2}
    = m_k^2 \sqrt{d}.
  \end{align*}

  For the second term,
  \begin{align*}
    \E[\max_i \norm{Z_iZ_i^T - I}^{k/2}]^{2/k}
    &\leq n^{2/k} \E[\norm{Z Z^T - I}^{k/2}]^{2/k} \\
    &= n^{2/k} \E[|\norm{Z}^2 - 1|^{k/2}]^{2/k} \\
    &\leq n^{2/k} (1 + \E[\norm{Z}^k]^{2/k}) \\
    &\leq n^{2/k} (1 + m_k^2 d).
  \end{align*}
  Thus,
  \begin{align*}
    \E\left[\Big\|\sum_{i=1}^n (Z_iZ_i^T - I)\Big\|^{k/2}\right]^{2/k}
    &\leq m_k^2 \sqrt{\frac{eknd}{2}}
      + ekn^{2/k}(1 + m_k^2 d)
    = O\left(m_k^2[\sqrt{kdn} + kdn^{2/k}]\right)
  \end{align*}
  and
  \begin{align*}
    \P(\big\|\hat{\Sigma} - I\big\| \geq \alpha)
    = (\alpha n)^{-k/2} O\left(m_k^2[\sqrt{kdn} + kdn^{2/k}]\right)^{k/2} \\
    = O\left(\alpha^{-1} m_k^2[\sqrt{kd/n} + kdn^{2/k-1}]\right)^{k/2}
  \end{align*}
  Choosing $\alpha \asymp m_k^2 \delta^{-2/k} \max\{\sqrt{k d}n^{-1/2}, k d n^{2/k-1}\} $,
  yields the desired probability bound of $\delta$.
\end{proof}

\begin{lemma}[Norm-boundedness]\label{lemma:k-moment-norm-boundedness}
  With probability at least $1-\delta$,
   $\bnorm^2 = m_k^2 d \delta^{-2/k} n^{2/k}$ for moment bounded
  data.
\end{lemma}
\begin{proof}
  By Lemma~\ref{lem:bdd-emp-cov-conc},
  $\norm{\Sigma^{-1}} \leq 2$ with probability at least ....
  Under this event all $i \in [n]$,
  $Z_i^T \hat{\Sigma}^{-1} Z_i \leq 2\norm{Z_i}^2$, and so it suffices to bound
  the $\ell_2$ norms of each data point.
  
  Then, for $B > 0$,
  \begin{align*}
    \P(\norm{Z}^2 > B)
    \leq B^{-k/2}\E[\norm{Z}^k]
    \leq m_k^k d^{k/2} B^{-k/2}.
  \end{align*}
  By picking $B = m_k^2 d \left(\frac{n}{\delta}\right)^{2/k}$,
  we have this is bounded by probability $\frac{\delta}{n}$.
\end{proof}

\begin{lemma}[Inner product concentration]\label{lemma:inner-product-concentration}
  % Let $X_1, \dots, X_n$ be i.i.d. mean zero and isotropic subgaussian
  % random vectors in $\R^d$.
  % Let $\hat{\Sigma} = \frac{1}{n} \sum_{i=1}^n Z_i Z_i^T$.
  With probability at least $1-\delta$,
  for all distinct $i, j \in [n]$,
  \begin{align*}
    |Z_i^T \hat{\Sigma}^{-1} Z_j| \leq 2m_k\delta^{-1/k}n^{2/k}\sqrt{2\bnorm^2}.
  \end{align*}
\end{lemma}
\begin{proof}
  The same argument as in the subgaussian case goes through except that with
  probability $1-\beta$, we have that
  \begin{align*}
    |Z_i^T \hat{\Sigma}_{-i}^{-1} Z_j| \leq
    m_k\beta^{-1/k}\norm{\hat{\Sigma}_{-i}^{-1/2}} \norm{\hat{\Sigma}_{-i}^{-1/2} Z_j}.
  \end{align*}
  Using this while keeping the rest of the argument the same, gives the result
\end{proof}

\begin{lemma}[Operator norm resilience]\label{lem:heavy-op-norm-resilience}
  Suppose $Z_1, \dots, Z_n$ are i.i.d. mean zero and isotropic with $k$
  moment bounded by $m_k$.
  Let $\delta > 0$ and $m \leq n$ such that $d + \log(1/\delta) = o(m)$.
  With probability at least $1-2\delta$,
  we have for all $v \in \S^{d-1}$ and all $T \subseteq [n]$ such that
  $|T| = m$ that
  \begin{align*}
    \frac{1}{n}\sum_{i \in T} (Z_i \cdot v)^2
    \lesssim
      m_k^2 \max\{\sqrt{k}n^{-1/2}, kn^{2/k-1}\} \delta^{-2/k}
      + m_k^2 \left(\sqrt{\frac{d + \log(2/\delta)}{n}}
        + \left(\frac{m}{n}\right)^{1-2/k}\right).
  \end{align*}
\end{lemma}
\begin{proof}
  By Lemma~\ref{lem:bdd-emp-cov-conc}
  \begin{align*}
    \norm{\hat{\Sigma} - I}
    = O\left(m_k^2 \delta^{-2/k} \max\{\sqrt{k d}n^{-1/2}, k d n^{2/k-1}\}\right),
  \end{align*}
  with probability at least $1-\delta$.
  Under this event, we prove the claim.
  It suffices to bound, for each $v$ in a $\frac{1}{2}$-packing of $\S^{d-1}$
  (which has size $\exp(O(d))$),
  the quantity that
  \begin{align*}
    Y_v := \sup_{\substack{T \subseteq [n] \\ |T|=m}}
      \frac{1}{n}\sum_{i \in T} (Z_i \cdot v)^2
  \end{align*}
  with probability at least $1-\delta e^{-O(d)}$.
  We will bound this using Propostion 3.4 of \url{https://arxiv.org/pdf/2209.13485}.
  Using the notation of this paper,
  we let $W_i = (Z_i \cdot v)^2$ and observe that
  \begin{align*}
    Y_v &= \sup_{\substack{T \subseteq [n] \\ |T|=m}}
    \frac{1}{n}\sum_{i \in T} (Z_i \cdot v)^2 \\
    &= \frac{1}{n} \sum_{i \in [n]} (Z_i \cdot v)^2
      - \inf_{\substack{T \subseteq [n] \\ |T|=n-m}}
        \frac{1}{n}\sum_{i \in T} (Z_i \cdot v)^2 \\
    &= T_0 - \frac{n-m}{n} \cdot T_{m} \\
    &= T_0 - 1 - \frac{n-m}{n} \cdot (T_m - 1) + \frac{m}{n},
  \end{align*}
  where $T_0$ and $T_m$ are again from the notation of that paper.
  Thus,
  \begin{align*}
    Y_v \leq |T_0 - 1| + |T_m - 1| + \frac{m}{n}.
  \end{align*}
  To bound the first term, we have
  \begin{align*}
    |T_0 - 1| = |v^T \hat{\Sigma} v - 1|
    \leq \norm{\hat{\Sigma} - I}
    \leq \alpha.
  \end{align*}
  Now to bound the second term, we have by Proposition 3.4 that
  with probability at least $1-\beta$,
  \begin{align*}
    |T_m - 1|
    &\lesssim \sqrt{\frac{\E[(Z_1 \cdot v)^2]\log(2/\beta)}{n}}
      + \E[|Z_1 \cdot v|^{k}]^{2/k}\left(\frac{m}{n}\right)^{1 - 2/k} \\
    &\leq m_k^2 \left(\sqrt{\frac{\log(2/\beta)}{n}} + \left(\frac{m}{n}\right)^{1-2/k}\right).
  \end{align*}
  Picking $\beta = \delta e^{-O(d)}$ and plugging it all in yields,
  \begin{align*}
    Y_v
    \lesssim
      m_k^2 \max\{\sqrt{k}n^{-1/2}, kn^{2/k-1}\} \delta^{-2/k}
      + m_k^2 \left(\sqrt{\frac{d + \log(2/\delta)}{n}}
        + \left(\frac{m}{n}\right)^{1-2/k}\right)
      + \frac{m}{n}
  \end{align*}

\end{proof}
% \begin{proof}OLD

%   \begin{align*}
%     \P(\norm{X} \geq M)
%     &\leq M^{-k} \E[\norm{X}^k] \\
%     &= M^{-k} \E\left[\left(\sum_{j=1}^d (X \cdot e_j)^2\right)^{k/2}\right] \\
%     &= d^{k/2} M^{-k}
%       \E\left[\left(\frac{1}{d}\sum_{j=1}^d (X \cdot e_j)^2\right)^{k/2}\right] \\
%     &\leq d^{k/2} M^{-k}
%       \E\left[\frac{1}{d}\sum_{j=1}^d |X \cdot e_j|^k\right] \\
%     &\leq (C\sqrt{d}/M)^k
%   \end{align*}

%   \begin{align*}
%     \E[(X\cdot v)^2] - \E[(X' \cdot v)^2]
%     &= \E[(X\cdot v)^2 \1{\norm{X} \geq M}] \\
%     &\leq \E[|X\cdot v|^k]^{\frac{2}{k}} \P(\norm{X} \geq M)^{1 - \frac{2}{k}}  \\
%     &\leq C^2 \P(\norm{X} \geq M)^{1 - \frac{2}{k}} \\
%     &\leq C^k \left(\frac{\sqrt{d}}{M}\right)^{k-2}
%   \end{align*}

%   \begin{align*}
%     &\P(\norm{\sum X_i X_i^T \1{\norm{X_i} \geq B}} \geq n\alpha) \\
%     &= \P(\norm{\sum X_i X_i^T \1{\norm{X_i} \geq B}}^{k/2} \geq (n\alpha)^{k/2}) \\
%     &\leq (n\alpha)^{-k/2}\E[\norm{\sum X_i X_i^T \1{\norm{X_i} \geq B}}^{k/2}] \\
%     &\leq (n\alpha)^{-k/2}\left(\sqrt{n} \E[\norm{XX^T\1{\norm{X} \geq B}}]^{1/2} + \sqrt{2ek}(n\E[\norm{XX^T}^{k/2}\1{\norm{X} \geq B}])^{1/k}\right)^k \\
%     &\leq (n\alpha)^{-k/2}\left(\sqrt{n} \E[\norm{X}^2\1{\norm{X} \geq B}]^{1/2} + \sqrt{2ek}(n\E[\norm{X}^k\1{\norm{X} \geq B}])^{1/k}\right)^k \\
%     &\leq (n\alpha)^{-k/2}\left(\sqrt{n} \E[\norm{X}^k]^{1/k}\P(\norm{X} \geq B)^{\frac{1}{2}-\frac{1}{k}} + \sqrt{2ek}(n\E[\norm{X}^k\1{\norm{X} \geq B}])^{1/k}\right)^k \\
%   \end{align*}


%   We need to show that with probability at least $1 - \exp(\Omega(\alpha^2 n))$
%   that for all
%   $v \in \S^{d-1}$,
%   \begin{align*}
%     \sup_{T \subseteq [n]} \frac{1}{n} \sum_{i \in T} (X_i \cdot v)^2
%     = v^T \left[\frac{1}{n} \sum_{i \in T} X_i X_i^T\right] v
%     \leq 4 \alpha.
%   \end{align*}


%   \begin{claim}
%     Let $\cV$ be a $\delta$-net of $\S^{d-1}$ and let $A$ be a PSD matrix.
%     If $v^T A v \leq M$ for all $v \in \cV$, then $\norm{A} \leq \frac{M}{1-\delta^2}$.
%   \end{claim}
%   \begin{proof}[Proof of claim]
%     Pick $v \in \S^{d-1}$ such that
%     $v^T A v = \norm{A}$.
%     Then there exists $w \in \cV$ such that $\norm{v - w} \leq \delta$.
%     We then have
%     \begin{align*}
%       w^T A w
%        & = v^T A v + 2(w - v)^T A v + (v - w)^T A (v - w)                             \\
%        & \geq v^T A v - 2\sqrt{(w - v)^T A (w-v)}\sqrt{v^T A v} + (w - v)^T A (w - v) \\
%        & = (\sqrt{v^T A v} - \sqrt{(v - w)^T A (v-w)})^2                              \\
%        & \geq (1-\delta^2) \norm{A}.
%     \end{align*}
%     Because $w \in \cV$, $w^T A w \leq M$, and so rearranging yields the desired result.
%   \end{proof}

%   Let $\cV$ be a $\frac{1}{2}$-net of $\S^{d-1}$ with size $|\cV| = \exp(O(d))$.
%   By applying a union bound over $\cV$, it suffices to show for
%   $v \in \cV$ that with probability at least
%   $1 - \exp(-\Omega(\alpha^2 n)-O(d)) = 1 - \exp(-\Omega(\alpha^2 n))$,
%   \begin{align*}
%     \sup_{T \subseteq [n]} \frac{1}{n} \sum_{i \in T} (X_i \cdot v)^2
%     = v^T \left[\frac{1}{n} \sum_{i \in T} X_i X_i^T\right] v
%     \leq \alpha I.
%   \end{align*}
%   For a fixed $v \in \cV$, let $Y_i = (X_i \cdot v)^2$.
%   We then have that the $Y_i$ are i.i.d. with expectation $1$ and
%   $\E[Y_i^{k/2}] \leq C^k$.
%   Now recall $B = ...$.
%   We have
%   \begin{align*}
%     \sup_{T \subseteq [n]} \frac{1}{n} \sum_{i \in T} Y_i
%      & \leq \sup_{T \subseteq [n]} \frac{1}{n} \sum_{i \in T} Y_i \1{Y_i \leq B}
%     + \frac{1}{n} \sum_{i=1}^n Y_i \1{Y_i > B}                                   \\
%      & \leq \frac{mB}{n} + \frac{1}{n} \sum_{i=1}^n Y_i \1{Y_i > B}.             \\
%      & \leq \frac{\alpha}{4} + \frac{1}{n} \sum_{i=1}^n Y_i \1{Y_i > B}.
%   \end{align*}
%   We now bound $\frac{1}{n} \sum_{i=1}^n Y_i \1{Y_i > B}$ with high probability.
%   Let $m = \E[Y_i \1{Y_i > B}]$.
%   We have that
%   \begin{align*}
%     m
%     &= \E[Y_i \1{Y_i > B}] \\
%     &= \int_0^\infty \P(Y_i \1{Y_i > B} > t) dt  \\
%     &= \int_0^\infty \P(Y_i > \max\{t, B\}) dt \\
%     &\leq \int_0^\infty \frac{C^k}{\max\{t, B\}^{k/2}}dt \\
%     &= C^k\left[\int_0^B \frac{1}{B^{k/2}} dt + \int_B^\infty \frac{1}{t^{k/2}} dt\right] \\
%     &= \frac{k}{k-2} \cdot \frac{C^k}{B^{k/2-1}}
%     \leq \frac{\alpha}{2},
%   \end{align*}
%   by our choice of $B$.
%   Then because $Y_i \1{Y_i > B}$ has $k/2$ moments
%   \begin{align*}
%     \P\left(\frac{1}{n} \sum_{i=1}^n [Y_i \1{Y_i > B}- m] \geq \frac{\alpha}{4}\right)
%      & = \P\left(\sum_{i=1}^n [Y_i \1{Y_i > B} - m] \geq \frac{\alpha n}{4}\right)               \\
%      & \leq \exp\left(-c \min\left\{\frac{(\alpha n)^2}{16 n}, \frac{\alpha n}{4}\right\}\right) \\
%      & = \exp(-c\alpha^2 n).
%   \end{align*}
%   Thus, with probability at least $1 - \exp(-\Omega(\alpha^2 n))$, we have
%   \begin{align*}
%     \sup_{T \subseteq [n]} \frac{1}{n} \sum_{i \in T} Y_i
%      & \leq \alpha,
%   \end{align*}
%   as desired.
% \end{proof}

% \subsubsection{Inner product resilience}
% \begin{lemma}[Inner product concentration]\label{lemma:inner-product-concentration}
%   Let $X_1, \dots, X_n$ be i.i.d. mean zero and isotropic subgaussian
%   random vectors in $\R^d$.
%   Let $\hat{\Sigma} = \frac{1}{n} \sum_{i=1}^n X_i X_i^T$.
%   Then with high probability,
%   for all distinct $i, j \in [n]$,
%   \begin{align*}
%     |X_i^T \hat{\Sigma}^{-1} X_j| \leq \ti{O}(\sqrt{d}).
%   \end{align*}
% \end{lemma}
% \begin{proof}
%   Let $\hat{\Sigma}_{-ij} = \frac{1}{n} \sum_{k \neq i,j} X_k X_k^T$.
%   Then we have that
%   \begin{align*}
%     \hat{\Sigma}^{-1}
%      & = (\hat{\Sigma}_{-j} + \frac{1}{n}X_jX_j^T)^{-1} \\
%      & = \hat{\Sigma}_{-j}^{-1}
%     - \frac{1}{n(1 - \frac{1}{n}X_j^T\hat{\Sigma}_{-j}^{-1}X_j)}
%     \hat{\Sigma}_{-j}^{-1} X_j X_j^T \hat{\Sigma}_{-j}^{-1},
%   \end{align*}
%   which implies
%   \begin{align*}
%     X_i^T \hat{\Sigma}^{-1} X_j
%      & = \left(1 - \frac{X_j^T\hat{\Sigma}_{-j}^{-1}X_j}
%     {n - X_j^T\hat{\Sigma}_{-j}^{-1}X_j}\right)
%     X_i^T \hat{\Sigma}_{-j}^{-1} X_j
%     = (1-o(1))X_i^T \hat{\Sigma}_{-j}^{-1} X_j.
%   \end{align*}
%   Now, we have that
%   \begin{align*}
%     \hat{\Sigma}_{-j}^{-1}
%      & = (\hat{\Sigma}_{-ij} + \frac{1}{n}X_iX_i^T)^{-1} \\
%      & = \hat{\Sigma}_{-ij}^{-1}
%     - \frac{1}{n(1 - \frac{1}{n}X_i^T\hat{\Sigma}_{-ij}^{-1}X_i)}
%     \hat{\Sigma}_{-ij}^{-1} X_i X_i^T \hat{\Sigma}_{-ij}^{-1},
%   \end{align*}
%   which implies
%   \begin{align*}
%     X_i^T \hat{\Sigma}^{-1} X_j
%      & = \left(1 - \frac{X_i^T\hat{\Sigma}_{-ij}^{-1}X_i}
%     {n - X_i^T\hat{\Sigma}_{-ij}^{-1}X_i}\right)
%     X_i^T \hat{\Sigma}_{-ij}^{-1} X_j
%     = (1-o(1))X_i^T \hat{\Sigma}_{-ij}^{-1} X_j.
%   \end{align*}
%   Thus, it suffices to show that with probability at least ...,
%   $|X_i^T \hat{\Sigma}_{-ij}^{-1} X_j| \leq \ti{O}(\sqrt{d})$.

%   With high probability over the randomness of $X_k$ for $k \neq i,j$,
%   $\norm{\hat{\Sigma}_{-ij}^{-1}} \leq 2$.
%   Then with high probability over the randomness of $X_i$,
%   $\norm{\hat{\Sigma}_{-ij}^{-1} X_i} \leq \ti{O}(\sqrt{d})$.
%   Finally, with high probability over the randomness of $X_j$,
%   $X_j$ is $\ti{O}(1)$ mass in the direction of $\hat{\Sigma}_{-ij}^{-1} X_i$,
%   proving the claim.
% \end{proof}

% % \begin{lemma}[Inner-product resilience to subtractive contamination]\label{lemma:inner-prod-subtractive}
% %   Let $X_1, \dots, X_n$ be i.i.d. mean zero and isotropic subgaussian
% %   random vectors in $\R^d$.
% %   Let $\hat{\Sigma} = \frac{1}{n} \sum_{i=1}^n X_i X_i^T$.
% %   Let $T \subseteq [n]$ be a set of indices such that $|B| \leq \eps n$.
% %   Let $\Sigma_B = \frac{1}{n} \sum_{i \in B} X_i X_i^T$.
% %   Then with high probability,
% %   for all distinct $i, j \in [n] \setminus B$,
% %   \begin{align*}
% %     |X_i^T (\hat{\Sigma} - \Sigma_B)^{-1} X_j| \leq \ti{O}(\sqrt{d}).
% %   \end{align*}
% % \end{lemma}

==> sections/goodness.tex <==
\section{Performance of $\alg$ for i.i.d. data}


\input{sections/goodness-subg}

\input{sections/goodness-kmom}

==> sections/pf-few-good-pts-in-S.tex <==
\subsection{Proof of Lemma~\ref{lemma:few-good-points-in-S}}
\label{sec:pf-good-pts-in-S}
Recall that in our notation, for an arbitrary dataset $\cY = \{y_1, \dots, y_m\}
  \subset \R^d$, we denote $\scov{\ds}{} = \frac{1}{m}\sum_{i=1}^m y_iy_i^T$.
Moreover, for subsets $T \subseteq [m]$, we denote
$\scov{\ds}{T} = \frac{1}{m}\sum_{i \in T} y_i y_i^T$.

\begin{lemma}\label{lem:bound-large-norms}
  Let $\cY = \{y_1, \dots, y_m\} \subset \R^d$ such that for all $i \in [m]$,
  $y_i^T \scovinv{\ds}{} y_i \leq M^2$.
  Also let $\gamma, b > 0$, $T \subseteq [m]$ and
  $\cW = \{w_1, \dots, w_k\} \subset \R^d$ be such that
  $\Sigma^{\cW} \preceq \frac{\gamma m}{k}\scov{\ds}{T}$ and for all $j \in [k]$,
  $w_j^T \big(\scovinv{\ds}{T} - \scovinv{\ds}{}\big) w_j \geq b$.
  Then $k \leq \frac{\gamma M^2}{b}(m - |T|)$.
\end{lemma}
\begin{proof}
  Let $\Sigma = \scov{\ds}{}$ for convenience.
  Because $T \subseteq [m]$, we have that $\Sigma_T \preceq \Sigma$ and so
  for all $j \in [k]$, it holds that
  $w_j^T (\Sigma_{T}^{-1} - \Sigma^{-1})w_j \geq 0$.

  Let $J \sim \uniform([k])$ so that we have
  $\E[w_J w_J^T] = \Sigma^{\cW}$.
  Then because $w_J^T (\Sigma_T^{-1} - \Sigma^{-1}) w_J \geq b$ almost surely,
  so we have by Markov's inequality that
  \begin{align*}
    1
     & = \P(w_J^T (\Sigma_T^{-1} - \Sigma^{-1}) w_J \geq b)                    \\
     & \leq \frac{1}{b} \E[w_J^T (\Sigma_T^{-1} - \Sigma^{-1}) w_J]            \\
     & = \frac{1}{b} \tr((\Sigma_T^{-1} - \Sigma^{-1})\Sigma^{\cW})            \\
     & \leq \frac{\gamma m}{k b} \tr((\Sigma_T^{-1} - \Sigma^{-1})\Sigma_{T}),
  \end{align*}
  Which implies $k \leq \frac{\gamma m}{b} \tr((\Sigma_T^{-1}-\Sigma^{-1})\Sigma_T)$.
  % This means at most $\frac{\gamma n}{b}\tr((\Sigma_T^{-1} - \Sigma^{-1})\Sigma_T)$
  % points $i \in T'$ have $y_i^T (\Sigma_T^{-1} - \Sigma^{-1}) y_i \geq b$.
  To bound the trace, we have that
  \begin{align*}
    \tr((\Sigma_T^{-1} - \Sigma^{-1})\Sigma_T)
    = \tr(I - \Sigma^{-1}\Sigma_T)
    = \tr(\Sigma^{-1}(\Sigma - \Sigma_T)).
  \end{align*}
  Noting that $\Sigma - \Sigma_T
    = \scov{\ds}{} - \scov{\ds}{T}
    = \frac{1}{m} \sum_{i \in [m] \setminus T} y_i y_i^T$,
  we have
  \begin{align*}
    \tr(\Sigma^{-1}(\Sigma - \Sigma_T))
     & = \frac{1}{m} \sum_{i \in [m] \setminus T} y_i^T \Sigma^{-1} y_i
    \leq \frac{M^2(m-|T|)}{m},
  \end{align*}
  proving the claim.
\end{proof}

% \begin{lemma}
%   $|G \cap S| = O(\eps + \eps^2 d) \cdot n$.
% \end{lemma}
% \begin{proof}
%   % Every iteration, two points $x, y \not\in S$ are added to $S$.
%   The number of points in $G$ that were added to $S$ along with a point in $B$
%   is clearly at most $|B| = \eps n$.
%   Thus, we bound the number of times that two points in $G$ were added to $S$
%   together.

%   WLOG take $\Sigma_G = I$, so that $\Sigma = I + \Sigma_B$.
%   Define the residual covariance matrix $M := I - \Sigma^{-1} \succeq 0$
%   and let $G' = \{x \in G \mid x^T M x \gtrsim 1/\eps\}$.
%   Then, for two points $x, y \in G$ to be added to $S$ together, we must have
%   \begin{align*}
%     1/\eps \leq |x^T\Sigma^{-1}y|
%     \leq |x^Ty| + |x^T M y|
%     = O(\sqrt{d} + \sqrt{x^T M x} \sqrt{y^T M y}).
%   \end{align*}
%   This implies that
%   \begin{align*}
%     \max\{x^T M x, y^T M y\} \gtrsim 1/\eps,
%   \end{align*}
%   and so at least one of $x$ and $y$ must be in $G'$.
%   Therefore, the result follows after showing $|G'| = O(\eps^2 d) n$.
%   To this end, let $X \sim G$ and note that
%   \begin{align*}
%     \P(X^T M X \gtrsim 1/\eps)
%     \lesssim \eps \E[X^T M X]
%     = \eps \tr(M \Sigma_G)
%     \lesssim \eps^2 d.
%   \end{align*}
%   [TODO: Show that $\tr(M) = O(\eps d)$]
% \end{proof}

% \begin{lemma}[Attempt 2]
%   $|G \cap S| = O(\eps + \eps^2 d) \cdot n$.
% \end{lemma}
% \begin{proof}
%   Similar to how $\Sigma_T = \frac{1}{n} \sum_{i \in T} x_i x_i^T$,
%   let $\hat{\Sigma}_T = \frac{1}{n} \sum_{i \in T} z_i z_i^T$; that is,
%   the covariance on the uncorrupted data.
%   Also let $\hat{\Sigma} = \hat{\Sigma}_{[n]}$.

%   % Every iteration, two points $x, y \not\in S$ are added to $S$.
%   The number of points in $G$ that were added to $S$ along with a point in $B$
%   is clearly at most $|B| = \eps n$.
%   Thus, we bound the number of times that two points in $G$ were added to $S$
%   together.

%   Let $M = \hat{\Sigma}^{-1} - \Sigma_R^{-1}$
%   and let $G' = \{i \in [n] \mid |z_i^T M z_i| \geq \frac{1}{\eps}\}$.
%   For two points $x, y \in G$ to be added to $S$ together, we must have
%   \begin{align*}
%     1/\eps \leq |x^T\Sigma_R^{-1}y|
%     \leq |x^T \hat{\Sigma}^{-1} y| + |x^T M y|
%     = O(\sqrt{d} + \sqrt{x^T M x} \sqrt{y^T M y}).
%   \end{align*}
%   This implies that
%   \begin{align*}
%     \max\{x^T M x, y^T M y\} \gtrsim 1/\eps,
%   \end{align*}
%   and so at least one of $x$ and $y$ must be in $G'$.
%   Therefore, the result follows after showing $|G'| = O(\eps^2 d) n$.
%   To this end, let $i \sim [n]$ and note that
%   \begin{align*}
%     \P(z_i^T M z_i \gtrsim 1/\eps)
%     \lesssim \eps \E[z_i^T M z_i]
%     = \eps \tr(M \hat{\Sigma})
%     = \eps \tr((\hat{\Sigma}^{-1} - \Sigma_R^{-1})\hat{\Sigma})
%     = \eps \cdot \tr(I - \Sigma_R^{-1}\hat{\Sigma}).
%   \end{align*}
%   Now notice that $\Sigma_R = \hat{\Sigma} - \hat{\Sigma}_{[n] \setminus G} + \Sigma_B$.
%   Then, letting
%   $\Delta = \hat{\Sigma}^{-1/2}( \hat{\Sigma}_{[n] \setminus G} - \Sigma_B)\hat{\Sigma}^{-1/2}$,
%   we have that
%   \begin{align*}
%     \P(z_i^T M z_i \gtrsim 1/\eps)
%     \lesssim \eps \cdot \tr(I - (I - \Delta)^{-1})
%     = O(\eps \tr(\Delta))
%     = O(\eps^2 d).
%   \end{align*}
% \end{proof}

% \begin{lemma}
%   Suppose $\Delta$ is a symmetric matrix such that $\lambda_{\min}(\Delta) \geq -1/2$.
%   Then for any vectors $x, y$,
%   \begin{align*}
%     |x^T (I+\Delta)^{-1} y| \leq |x^T y| + 2 \sqrt{x^T|\Delta|x} \sqrt{y^T|\Delta|y},
%   \end{align*}
%   where $|\Delta|$ is $\Delta$ with absolute values applied to the eigenvalues.
% \end{lemma}
% \begin{proof}
%   Suppose without loss of generality that $\Delta$ is diagonal.
%   Then we have that
%   \begin{align*}
%     |x^T (I+\Delta)^{-1} y|
%     &= \left| \sum_{k=1}^d \frac{x_k y_k}{1+\Delta_{kk}} \right| \\
%     &\leq \left| \sum_{k=1}^d x_k y_k \right|
%       + \sum_{k=1}^d \left| \frac{\Delta_{kk}}{1+\Delta_{kk}}\right| |x_k| |y_k|  \\
%     &\leq |x^Ty|
%       + 2\sum_{k=1}^d \left| \Delta_{kk}\right| |x_k| |y_k|.
%   \end{align*}
%   The result then follows by Cauchy-Schwarz.
% \end{proof}

\begin{lemma}[Restatement of Lemma~\ref{lemma:few-good-points-in-S}]
  %<*few-good-pts-in-S-lemma>
  Suppose $\tinner \geq 2\binner$, $\tnorm \geq \bnorm$, and
  $|[n] \setminus (G \cap \Rnorm)| \leq \min\{\mop, \frac{n}{4}\}$.
  Then we have
  \begin{align*}
    |G \cap S|
    \leq 2\mbig + |B \cap \Rnorm|
    + \frac{72 \tnorm^2}{\tinner} (n-|G \cap \Rnorm|).
  \end{align*}
  %</few-good-pts-in-S-lemma>
\end{lemma}
\begin{proof}
  Throughout this proof, we denote $\Rnorm$ as $R$ for ease of notation.

  Note that $S_1$ and $S_2$ partition $S$, $R_1$ and $R_2$ partition $R$,
  and $\Hone$ and $\Htwo$ partition $[n]$.
  Thus, it suffices to show that
  \begin{align*}
    |G \cap S_1|
     & \leq |B \cap R_1|
    + \frac{72\tnorm^2}{\tinner}(|\Htwo| - |G \cap R_2|),\mbox{ and} \\
    |G \cap S_2|
     & \leq |B \cap R_2|
    + \frac{72\tnorm^2}{\tinner}(|\Hone| - |G \cap R_1|).
  \end{align*}
  We will only show the first inequality, as the other inequality is symmetric.

  $\alg$ computes $S_1$ in Line~\ref{alg:compute-S-call-1}
  by calling $\computeS$.
  Within $\computeS$, points are added to $S_1$ in pairs during
  Lines~\ref{compS:loop-cond}-\ref{compS:loop-end}.
  Thus, for every $i \in S_1$, we may let $j(i) \in S_1$ be the other index
  that point $i$ was added alongside.
  Because the condition in Line~\ref{compS:loop-cond} of $\computeS$ prevents
  a point from being added more than once, we have that the choice of
  $j(i)$ is unique for each $i \in S_1$ and moreover,
  $j(i) \neq j(i')$ for distinct $i, i' \in S_1$.
  Also note that for $i \in S_1$, it must be the case that $i \in R_1$
  because otherwise the $i$th entry of $\cX_{R_1}$ is $0$, which has an
  inner product of 0 with every other data point and thus would not be added
  to $S_1$.

  To bound $|G \cap S_1|$, first observe that for each $i \in G \cap S_1$,
  either $j(i) \in B \cap S_1$ or $j(i) \in G \cap S_1$.
  By injectivity of $j(\cdot)$, there are at most $|B \cap S_1|$
  points $i \in G \cap S_1$ are such that $j(i) \in B \cap S_1$.
  Moreover, because $S_1 \subseteq R_1$, we have $|B \cap S_1| \leq |B \cap R_1|$,
  Therefore, all we need to show is
  \begin{align*}
    |\{i \in G \cap S_1 \mid j(i) \in G \cap S_1\}|
    \leq 2\mbig + \frac{72 \tnorm^2}{\tinner} (|\Htwo|-|G \cap R_2|).
  \end{align*}

  Now consider the set
  $Q = \{i \in G \cap S_1 \mid j(i) \in G \cap S_1,
    |x_i^T\scovinv{\uds}{\Htwo}x_{j(i)}| > \binner\}$.
  Because all of the pairs are disjoint elements of $(\Hone)^2$
  and because $\cZ$ is
  $(\mbig, \binner)$-inner product bounded,
  we immediately have that $|Q| \leq 2\mbig$.
  Thus, it only remains to show
  \begin{align*}
    |\{i \in G \cap S_1 \mid j(i) \in G \cap S_1,
    |x_i^T\scovinv{\uds}{\Htwo}x_{j(i)}| \leq \binner\}|
    \leq \frac{72 \tnorm^2}{\tinner} (|\Htwo|-|G \cap R_2|).
  \end{align*}

  Let $i \in G \cap S_1$ such that $j=j(i) \in G \cap S_1$
  and $|x_i^T\scovinv{\uds}{\Htwo}x_{j(i)}| \leq \binner$.
  Recall that in Line~\ref{alg:compute-S-call-1} of $\alg$, we call
  $\computeS$ with arguments $\cX_{R_1}$, $\Sigma_{R_2}^{-1}$, and $\tinner$;
  thus, we know by Line~\ref{compS:loop-cond} of $\computeS$ that
  $|x_i^T \scovinv{\cds}{R_2} x_j| > \tinner$.
  We can upper bound the inner product as
  \begin{align*}
    |x_i^T \scovinv{\cds}{R_2} x_j|
     & \leq \Big|x_i^T \scovinv{\uds}{\Htwo} x_j\Big|
    + \Big|x_i^T \Big(\scovinv{\cds}{G \cap R_2} - \scovinv{\uds}{\Htwo}\Big) x_j\Big|         \\
     & \qquad+ \Big|x_i^T \Big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2}\Big) x_j\Big|.
  \end{align*}
  The first term is bounded by $\binner$ by assumption.
  Now notice that
  $\scov{\cds}{G \cap R_2} = \scov{\uds}{G \cap R_2} \preceq \scov{\uds}{\Htwo}$ and
  $\scov{\cds}{G \cap R_2} \preceq \scov{\cds}{R_2}$, and so by applying Cauchy-Schwarz,
  \begin{align*}
    |x_i^T \scovinv{\cds}{R_2} x_j|
     & \leq \binner
    + \sqrt{x_i^T \Big(\scovinv{\cds}{G \cap R_2} - \scovinv{\uds}{\Htwo}\Big) x_i}
    \sqrt{x_j^T \Big(\scovinv{\cds}{G \cap R_2} - \scovinv{\uds}{\Htwo}\Big) x_j}          \\
     & \qquad+ \sqrt{x_i^T \Big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2}\Big) x_i}
    \sqrt{x_j^T \Big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2}\Big) x_j}.
  \end{align*}

  Combining this with the facts that
  $|x_i^T \scovinv{\cds}{R_2} x_j| > \tinner$ and $\binner \leq \frac{1}{2}\tinner$,
  we must have that
  \begin{enumerate}
    \item $x_i^T \big(\scovinv{\cds}{G \cap R_2} - \scovinv{\uds}{\Htwo}\big) x_i
            \geq \frac{1}{4}\tinner$; or
    \item $x_i^T \big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2}\big) x_i
            \geq \frac{1}{4}\tinner$; or
    \item $x_j^T \big(\scovinv{\cds}{G \cap R_2} - \scovinv{\uds}{\Htwo}\big) x_j
            \geq \frac{1}{4}\tinner$; or
    \item $x_j^T \big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2}\big) x_j
            \geq \frac{1}{4}\tinner$.
  \end{enumerate}

  Now define the sets
  \begin{align*}
    \Sgone & \defeq \big\{i \in G \cap R_1
    \mid x_i^T \big(\scovinv{\cds}{G \cap R_2} - \scovinv{\uds}{\Htwo}\big)x_i
    \geq \tfrac{1}{4}\tinner\big\},
    \\
    \Sgtwo & \defeq \big\{i \in G \cap R_1
    \mid x_i^T\big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2}\big) x_i
    \geq \tfrac{1}{4}\tinner\}.
  \end{align*}
  We have shown that for $i \in G \cap S_1$ such that $j(i) \in G \cap S_1$,
  either $i \in \Sgone \cup \Sgtwo$ or $j(i) \in \Sgone \cup \Sgtwo$.
  Because $j(\cdot)$ is injective, this allows to conclude that
  $|G \cap S_1| \leq 2|\Sgone \cup \Sgtwo| \leq 2|\Sgone| + 2|\Sgtwo|$.

  Before bounding $|\Sgone|$ and $|\Sgtwo|$, we first note that
  \begin{align*}
    |\Htwo \setminus (G \cap R_2)|
    \leq |[n] \setminus (G \cap R)|
    \leq \min\{\mop, \tfrac{n}{4}\},
  \end{align*}
  where the last inequality is by assumption.
  Then because $\cZ$ is $(\mop, \aop)$-operator norm resilient,
  we have by Lemma~\ref{lem:heavy-op-norm-resilience} that
  $\scov{\uds}{\Htwo} \preceq (1-\aop)^{-1} \scov{\uds}{G \cap R_2}$.

  Now to bound $|\Sgone|$, we will apply Lemma~\ref{lem:bound-large-norms} to
  $\cY = \cZ_{\Htwo}$, $T = G \cap R_2$, and
  $\cW = \cX_{\Sgone}$.
  Before doing so, we need the values of $M, C, b$ with which we can
  apply Lemma~\ref{lem:bound-large-norms} to these datasets.
  Because $\cZ$ is $\bnorm$-norm bounded, we have
  for all $i \in \Htwo$ that
  \begin{align*}
    z_i^T \scovinv{\ds}{} z_i
    = \frac{|\Htwo|}{n} z_i^T \scovinv{\uds}{\Htwo} z_i
    \leq \frac{1}{2}\bnorm^2,
  \end{align*}
  so we may take $M = \frac{1}{\sqrt{2}}\bnorm$.
  By definition of $\Sgone$, we have for $i \in \Sgone$ that
  \begin{align*}
    x_i^T\big(\scovinv{\ds}{T} - \scovinv{\ds}{})x_i
    = \frac{|\Htwo|}{n} x_i^T\big(\scovinv{\uds}{G \cap R_2} - \scovinv{\uds}{\Htwo})x_i
    \geq \frac{1}{8}\tinner,
  \end{align*}
  so we may take $b = \frac{1}{8}\tinner$.
  Finally, to find $\gamma$, we first note that because $\cZ$ is $(\mop, \aop)$-operator
  norm resilient, we have that
  $\scov{\uds}{\Hone} \preceq \frac{3}{4}\scov{\uds}{}$.
  Since $\scov{\uds}{} = \scov{\uds}{\Hone} + \scov{\uds}{\Htwo}$, this implies that
  $\scov{\uds}{\Hone} \preceq 3\scov{\uds}{\Htwo}$.
  Thus, because $\Sgone \subseteq \Hone$, we have
  \begin{align*}
    \Sigma^{\cW} = \frac{n}{|\Sgone|} \scov{\uds}{\Sgone}
    \preceq \frac{n}{|\Sgone|} \scov{\uds}{\Hone}
    \preceq \frac{3n}{|\Sgone|} \scov{\uds}{\Htwo}
    \preceq \frac{3n}{(1-\aop)|\Sgone|} \scov{\uds}{G \cap R_2}
    = \frac{3|\Htwo|}{(1-\aop)|\Sgone|} \scov{\ds}{T},
  \end{align*}
  and so we may take $\gamma = 3(1-\aop)^{-1}$.
  Applying Lemma~\ref{lem:bound-large-norms} with these quantities, we can
  conclude that
  $|\Sgone|
    \leq \frac{3}{1-\aop} \cdot \frac{\bnorm^2}{2} \cdot \frac{8}{\tinner} \cdot (|\Htwo| - |G \cap R_2|)
    \leq \frac{12\tnorm^2}{(1-\aop)\tinner}(|\Htwo| - |G \cap R_2|)$.

  To bound $|\Sgtwo|$, we will similarly apply
  Lemma~\ref{lem:bound-large-norms} to
  $\cY = \cX_{R_2}$, $T = G \cap R_2$, and
  $\cW = \cX_{\Sgtwo}$.
  Again, we need to compute the values of $M, C, b$ with which we can
  apply Lemma~\ref{lem:bound-large-norms} to these datasets.
  For $M$, we have by Lemma~\ref{lem:norm-filter-props} that for all $i \in R_2$,
  \begin{align*}
    x_i^T \scovinv{\ds}{} x_i
    = \frac{|R_2|}{n} x_i^T \scovinv{\cds}{R_2} x_i
    \leq \frac{1}{2}\tnorm^2,
  \end{align*}
  so we may take $M = \frac{1}{\sqrt{2}}\tnorm$.
  By definition of $\Sgtwo$, we have for $i \in \Sgtwo$ that
  \begin{align*}
    x_i^T\big(\scovinv{\ds}{T} - \scovinv{\ds}{})x_i
    = \frac{|R_2|}{n} x_i^T\big(\scovinv{\cds}{G \cap R_2} - \scovinv{\cds}{R_2})x_i
    \geq \frac{|R_2|}{4n}\tinner.
  \end{align*}
  Now note that
  \begin{align*}
    |R_2|
    \geq |G \cap R_2|
    = |\Htwo| - |\Htwo \setminus (G \cap R_2)|
    \geq \frac{n}{2} - \min\left\{\mop, \frac{n}{4}\right\}
    \geq \frac{n}{4},
  \end{align*}
  so we may take $b = \frac{1}{16}\tinner$.
  Finally, to find $\gamma$, by the same argument as when computed
  $\gamma$ for $|\Sgone|$, we have
  that $\Sigma^{\cW} \preceq \frac{3n}{(1-\aop)|\Sgtwo|} \scov{\uds}{G \cap R_2}
    =  \frac{3n}{(1-\aop)|\Sgtwo|} \scov{\cds}{G \cap R_2}
    = \frac{3|R_2|}{(1-\aop)|\Sgtwo|}\scov{\ds}{T}$,
  and so we may take $\gamma = 3(1-\aop)^{-1}$.
  Applying Lemma~\ref{lem:bound-large-norms} with these quantities, we can
  conclude that
  $|\Sgtwo|
    \leq \frac{3}{1-\aop} \cdot \frac{\tnorm^2}{2} \cdot \frac{16}{\tinner}
    \cdot (|R_2| - |G \cap R_2|)
    \leq \frac{24\tnorm^2}{\tinner}(|\Htwo| - |G \cap R_2|)$.

  Putting it all together, we have that
  $2|\Sgone| + 2|\Sgtwo| \leq \frac{72\tnorm^2}{(1-\aop)\tinner}(\Htwo - |G \cap R_2|)$,
  proving the claim.
\end{proof}


% \begin{lemma}[Restatement of Lemma~\ref{lemma:few-good-points-in-S}]
%   If $|G \setminus R| = O(\eps n)$,
%   then $|G \cap S| = \ti{O}(\eps + \eps^2 d) \cdot n$.
% \end{lemma}
% \begin{proof}
%   Similar to how $\Sigma_T = \frac{1}{n} \sum_{i \in T} x_i x_i^T$,
%   let $\hat{\Sigma}_T = \frac{1}{n} \sum_{i \in T} z_i z_i^T$; that is,
%   the covariance on the uncorrupted data.
%   Also let $\hat{\Sigma} = \hat{\Sigma}_{[n]}$.

%   % Every iteration, two points $x, y \not\in S$ are added to $S$.
%   The number of points in $G \cap R$ that were added to $S$ along with a point
%   in $B \cap R$ is clearly at most $|B| = \eps n$.
%   Thus, we bound the number of times that two points in $G \cap R$ were added to
%   $S$ together.

%   Then, let $G' = B \cup (G \setminus R)$ be the indices of good points missing from $R$.
%   By assumption, $|G'| = O(\eps n)$.
%   Now note that
%   \begin{align*}
%     \Sigma_R
%     = \hat{\Sigma} - \hat{\Sigma}_{G'} + \Sigma_{B \cap R},
%   \end{align*}
%   which implies
%   \begin{align*}
%     (\hat{\Sigma} + \Sigma_{B \cap R})^{-1}
%     \preceq \Sigma_R^{-1}
%     \preceq (\hat{\Sigma}-\hat{\Sigma}_{G'})^{-1}.
%   \end{align*}

%   For any $i, j \in G \cap R$, by the parallelogram law, we have that
%   \begin{align*}
%     4|x_i^T (\Sigma_R^{-1} - \hat{\Sigma}^{-1}) x_j|
%     & \leq |(x_i + x_j)^T (\Sigma_R^{-1} - \hat{\Sigma}^{-1}) (x_i + x_j)|
%       + |(x_i - x_j)^T (\Sigma_R^{-1} - \hat{\Sigma}^{-1}) (x_i - x_j)|.
%   \end{align*}
%   Define
%   $E_1 = (\hat{\Sigma}-\hat{\Sigma}_{G'})^{-1} - \hat{\Sigma}^{-1}$
%   and
%   $E_2 = \hat{\Sigma}^{-1} - (\hat{\Sigma} + \Sigma_{B \cap R})^{-1}$.
%   Notice that $E_1, E_2 \succeq 0$.
%   Then, the first term in the above display is bounded by
%   $\max\{(x_i+x_j)^TE_1(x_i+x_j), (x_i+x_j)^TE_2(x_i+x_j)\}
%     = O(\max\{x_i^T E_1 x_i, x_j^T E_1 x_j, x_i^T E_2 x_i, x_j^T E_2 x_j\})$.
%   By a similar reasoning, the latter bound also applies to the second term.

%   Now define $S_G = \{k \in [n] \mid z_k^T E_1 z_k \geq \frac{1}{\eps}\}$
%   and $S_B = \{k \in [n] \mid z_k^T E_2 z_k \geq \frac{1}{\eps}\}$.
%   The above calculations implies that, for any $i,j \in G'$ such that
%   $|x_i \Sigma_R^{-1} x_j| \geq \frac{1}{\eps}$, it must be the case that
%   either $i \in S_G \cup S_B$ or $j \in S_G \cup S_B$.
%   This implies that the number of good points that were added alongside
%   another good point is at most $2|S_G \cup S_B| \leq 2|S_G| + 2|S_B|$.

%   We now bound $|S_G|$.
%   Let $i \sim [n]$ and note that
%   \begin{align*}
%     \P(z_i^T E_1 z_i \gtrsim 1/\eps)
%      & \lesssim \eps \E[z_i^T E_1 z_i]                                                                       \\
%      & = \eps \tr(E_1 \hat{\Sigma})                                                                          \\
%      & = \eps \tr(((\hat{\Sigma}-\hat{\Sigma}_{G'})^{-1} - \hat{\Sigma}^{-1})\hat{\Sigma})       \\
%      & = \eps \cdot \tr((I - \hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2})^{-1} - I).
%   \end{align*}
%   Because $\norm{\hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2}} \leq 1/2$
%   due to operator norm resilience, we have that
%   \begin{align*}
%     \tr((I - \hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2})^{-1} - I)
%     \leq 2\tr(\hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2}).
%   \end{align*}

%   Then, expanding out $\hat{\Sigma}_{G'}$, we have
%   \begin{align*}
%     \tr(\hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2})
%      & = \frac{1}{n}\sum_{k \in G'} x_k^T \hat{\Sigma}^{-1} x_k
%     \leq \ti{O}(d|G'|/n)
%     = \ti{O}(\eps d),
%   \end{align*}
%   which thus implies $\P(z_k^T E_1 z_k \geq \frac{1}{\eps}) = \ti{O}(\eps^2 d)$
%   and hence $|S_G| = \ti{O}(\eps^2 d) n$.

%   Similarly, for $S_B$, we have that
%   \begin{align*}
%     \P(z_i^T E_2 z_i \gtrsim 1/\eps)
%     &\lesssim \eps \E[z_i^T E_2 z_i] \\
%     &= \eps \tr(E_2 \hat{\Sigma}) \\
%     &= \eps \tr((\hat{\Sigma}^{-1} - (\hat{\Sigma} + \Sigma_{B \cap R})^{-1})\hat{\Sigma}) \\
%     &= \eps \tr(\hat{\Sigma}^{-1}\Sigma_{B \cap R}(I+\hat{\Sigma}^{-1}\Sigma_{B \cap R})^{-1}) \\
%     &= \eps \tr(\Sigma_{B \cap R}(\hat{\Sigma}+\Sigma_{B \cap R})^{-1}) \\
%     &\leq \eps \tr(\Sigma_{B \cap R}(\Sigma_{G \cap R}+\Sigma_{B \cap R})^{-1}) \\
%     &= O(\eps^2 d).
%   \end{align*}

%   This proves the desired result.
% \end{proof}

% \begin{lemma}[Restatement of Lemma~\ref{lemma:few-good-points-in-S}]
%   If $|G \setminus R| = O(\eps n)$,
%   then $|G \cap S| = \ti{O}(\eps + \eps^2 d) \cdot n$.
% \end{lemma}
% \begin{proof}
%   Similar to how $\Sigma_T = \frac{1}{n} \sum_{i \in T} x_i x_i^T$,
%   let $\hat{\Sigma}_T = \frac{1}{n} \sum_{i \in T} z_i z_i^T$; that is,
%   the covariance on the uncorrupted data.
%   Also let $\hat{\Sigma} = \hat{\Sigma}_{[n]}$.

%   % Every iteration, two points $x, y \not\in S$ are added to $S$.
%   The number of points in $G \cap R$ that were added to $S$ along with a point
%   in $B \cap R$ is clearly at most $|B| = \eps n$.
%   Thus, we bound the number of times that two points in $G \cap R$ were added to
%   $S$ together.

%   First let $y_i = \Sigma_{G \cap R}^{-1/2} z_i$ be the whitened remaining good points.
%   Then, let $G' = B \cup (G \setminus R)$ be the indices of good points missing from $R$.
%   By assumption, $|G'| = O(\eps n)$.
%   Now note that
%   \begin{align*}
%     \Sigma_R
%     = \Sigma_{G \cap R} + \Sigma_{B \cap R},
%   \end{align*}
%   which implies
%   \begin{align*}
%     \Sigma_{G \cap R}^{-1/2}\Sigma_R \Sigma_{G \cap R}^{-1/2}
%     = I + \underbrace{
%       \Sigma_{G \cap R}^{-1/2}\Sigma_{B \cap R}\Sigma_{G \cap R}^{-1/2}
%     }_{=: \Delta}.
%   \end{align*}
%   Also let
%   $S = \{i \in [n] \mid |
%     x_i^T \hat{\Sigma}^{-1/2}\Delta \hat{\Sigma}^{-1/2} x_j| \geq \frac{1}{\eps}\}$.

%   We wish to apply the previous lemma with this $\Delta$, and for this we need
%   to show that $\lambda_{\min}(\Delta) \geq -1/2$.
%   Because $\Sigma_{B \cap R}$ and $\Sigma_G$ are both positive semidefinite,
%   it suffices to show that
%   $\norm{\hat{\Sigma}^{-1/2}\Sigma_{G'}\hat{\Sigma}^{-1/2}} \leq 1/2$.
%   This follows because $|G'| = O(\eps n) = o(n)$ and operator norm resilience
%   implies that $\Sigma_{G'} \preceq o(1) \hat{\Sigma}$.

%   Now, for any $i, j \in G \cap R$,
%   we may apply Lemma~ref{???} to see that
%   \begin{align*}
%     |y_i^T(I+\Delta)^{-1} y_j|
%     \leq |y_i^T y_j| +
%       \sqrt{y_i^T(I - (I+\Delta)^{-1}) y_i}
%       \sqrt{y_j^T(I - (I+\Delta)^{-1}) y_j}.
%   \end{align*}
%   [show that $|y_i^T y_j| = \ti{O}(\sqrt{d})$.]
%   This implies that if $|y_i^T (I+\Delta)^{-1} y_j| \geq \frac{1}{\eps}$,
%   then either $y_i^T(I - (I+\Delta)^{-1}) y_i \gtrsim \frac{1}{\eps}$ or
%   $y_i^T(I - (I+\Delta)^{-1}) y_i \gtrsim \frac{1}{\eps}$,
%   which implies either $i \in S$ or $j \in S$.

%   Therefore, we know that the number of good points removed with another good
%   point is at most $2|S|$, and so it suffices to bound $|S|$.
%   To do so, let $i \sim Uni(G \cap R)$ and note that
%   \begin{align*}
%     \P(y_i^T(I - (I+\Delta)^{-1}) y_i \gtrsim 1/\eps)
%     &\lesssim \eps \E[y_i^T(I - (I+\Delta)^{-1}) y_i] \\
%     &= \eps \tr(\Delta(I+\Delta)^{-1}) \\
%     &\leq \eps \tr(\Sigma_{B\cap R}\Sigma_R^{-1}) \\
%     &= O(\eps^2 d).
%   \end{align*}
%   % Then by the parallelogram law, we have that
%   % \begin{align*}
%   %   4|x_i^T (\Sigma_R^{-1} - \hat{\Sigma}^{-1}) x_j|
%   %   & \leq |(x_i + x_j)^T (\Sigma_R^{-1} - \hat{\Sigma}^{-1}) (x_i + x_j)|
%   %     + |(x_i - x_j)^T (\Sigma_R^{-1} - \hat{\Sigma}^{-1}) (x_i - x_j)|.
%   % \end{align*}
%   % Define
%   % $E_1 = (\hat{\Sigma}-\hat{\Sigma}_{G'})^{-1} - \hat{\Sigma}^{-1}$
%   % and
%   % $E_2 = \hat{\Sigma}^{-1} - (\hat{\Sigma} + \Sigma_{B \cap R})^{-1}$.
%   % Notice that $E_1, E_2 \succeq 0$.
%   % Then, the first term in the above display is bounded by
%   % $\max\{(x_i+x_j)^TE_1(x_i+x_j), (x_i+x_j)^TE_2(x_i+x_j)\}
%   %   = O(\max\{x_i^T E_1 x_i, x_j^T E_1 x_j, x_i^T E_2 x_i, x_j^T E_2 x_j\})$.
%   % By a similar reasoning, the latter bound also applies to the second term.

%   % Now define $S_G = \{k \in [n] \mid |z_k^T E_1 z_k| \geq \frac{1}{\eps}\}$
%   % and $S_B = \{k \in [n] \mid |z_k^T E_2 z_k| \geq \frac{1}{\eps}\}$.
%   % The above calculations implies that, for any $i,j \in G'$ such that
%   % $|x_i \Sigma_R^{-1} x_j| \geq \frac{1}{\eps}$, it must be the case that
%   % either $i \in S_G \cup S_B$ or $j \in S_G \cup S_B$.
%   % This implies that the number of good points that were added alongside
%   % another good point is at most $2|S_G \cup S_B| \leq 2|S_G| + 2|S_B|$.

%   % We now bound $|S_G|$.
%   % Let $i \sim [n]$ and note that
%   % \begin{align*}
%   %   \P(z_i^T E_1 z_i \gtrsim 1/\eps)
%   %    & \lesssim \eps \E[z_i^T E_1 z_i]                                                                       \\
%   %    & = \eps \tr(E_1 \hat{\Sigma})                                                                          \\
%   %    & = \eps \tr(((\hat{\Sigma}-\hat{\Sigma}_{G'})^{-1} - \hat{\Sigma}^{-1})\hat{\Sigma})       \\
%   %    & = \eps \cdot \tr((I - \hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2})^{-1} - I).
%   % \end{align*}
%   % Because $\norm{\hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2}} \leq 1/2$
%   % due to operator norm resilience, we have that
%   % \begin{align*}
%   %   \tr((I - \hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2})^{-1} - I)
%   %   \leq 2\tr(\hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2}).
%   % \end{align*}

%   This proves the desired result.
% \end{proof}

% \begin{lemma}[Restatement of Lemma~\ref{lemma:few-good-points-in-S}]
%   If $|G \setminus R| = O(\eps n)$,
%   then $|G \cap S| = \ti{O}(\eps + \eps^2 d) \cdot n$.
% \end{lemma}
% \begin{proof}
%   Similar to how $\Sigma_T = \frac{1}{n} \sum_{i \in T} x_i x_i^T$,
%   let $\hat{\Sigma}_T = \frac{1}{n} \sum_{i \in T} z_i z_i^T$; that is,
%   the covariance on the uncorrupted data.
%   Also let $\hat{\Sigma} = \hat{\Sigma}_{[n]}$.

%   % Every iteration, two points $x, y \not\in S$ are added to $S$.
%   The number of points in $G \cap R$ that were added to $S$ along with a point
%   in $B \cap R$ is clearly at most $|B| = \eps n$.
%   Thus, we bound the number of times that two points in $G \cap R$ were added to
%   $S$ together.

%   First let $y_i = \hat{\Sigma}^{-1/2} z_i$ be the whitened good points.
%   Then, let $G' = B \cup (G \setminus R)$ be the indices of good points missing from $R$.
%   By assumption, $|G'| = O(\eps n)$.
%   Now note that
%   \begin{align*}
%     \Sigma_R
%     = \hat{\Sigma} - \hat{\Sigma}_{G'} + \Sigma_{B \cap R},
%   \end{align*}
%   which implies
%   \begin{align*}
%     \hat{\Sigma}^{-1/2}\Sigma_R\hat{\Sigma}^{-1/2}
%     = I + \underbrace{
%       \hat{\Sigma}^{-1/2}(\Sigma_{B \cap R}
%       - \hat{\Sigma}_{G'})\hat{\Sigma}^{-1/2}
%     }_{=: \Delta}.
%   \end{align*}
%   Also let
%   $S' = \{i \in [n] \mid |
%     z_i^T \hat{\Sigma}^{-1/2}|I-(I+\Delta)^{-1}| \hat{\Sigma}^{-1/2} z_i| \geq \frac{1}{\eps}\}$.
%   % \begin{align*}
%   %   (\hat{\Sigma} + \Sigma_{B \cap R})^{-1}
%   %   \preceq \Sigma_R^{-1}
%   %   \preceq (\hat{\Sigma}-\hat{\Sigma}_{G'})^{-1}.
%   % \end{align*}

%   Now, for any $i, j \in G \cap R$,
%   \begin{align*}
%     |x_i^T \Sigma_R^{-1} x_j|
%     &\leq |z_i^T \hat{\Sigma}^{-1} z_j| + |z_i^T(\hat{\Sigma}^{-1} - \Sigma_R^{-1})z_j| \\
%     &= |z_i^T \hat{\Sigma}^{-1} z_j|
%       + |z_i^T\hat{\Sigma}^{-1/2}(I - (I+\Delta)^{-1})\hat{\Sigma}^{-1/2}z_j|.
%   \end{align*}
%   By bounded inner products of good points, we have that the first term is
%   $\ti{O}(\sqrt{d})$.
%   For the second term, we define $V = |I - (I+\Delta)^{-1}|$, where $|\cdot|$
%   refers to taking the matrix absolute value.
%   Then we use Cauchy-Schwarz to obtain,
%   \begin{align*}
%     |z_i^T\hat{\Sigma}^{-1/2}(I - (I+\Delta)^{-1})\hat{\Sigma}^{-1/2}z_j|
%     &\leq \sqrt{z_i^T\hat{\Sigma}^{-1/2}V\hat{\Sigma}^{-1/2}z_i}
%       \sqrt{z_j^T\hat{\Sigma}^{-1/2}V\hat{\Sigma}^{-1/2}z_j}. \\
%   \end{align*}
%   Thus, we have that if $|z_i^T \Sigma_R^{-1} z_j| \geq \frac{1}{\eps}$,
%   then either $i \in S'$ or $j \in S'$.
%   So we know that the number of good points removed with another good
%   point is at most $2|S'|$, and so it suffices to bound $|S'|$.
%   To do so, let $i \sim Uni([n])$ and note that
%   \begin{align*}
%     \P(z_i^T \hat{\Sigma}^{-1/2}|I-(I+\Delta)^{-1}| \hat{\Sigma}^{-1/2} z_i \geq \frac{1}{\eps})
%     &\lesssim \eps \E[z_i^T \hat{\Sigma}^{-1/2}|I-(I+\Delta)^{-1}| \hat{\Sigma}^{-1/2} z_i] \\
%     &= \eps \tr(\hat{\Sigma}^{-1/2}|I-(I+\Delta)^{-1}| \hat{\Sigma}^{-1/2} \hat{\Sigma}) \\
%     &= \eps \tr(|I-(I+\Delta)^{-1}|).
%   \end{align*}
%   Now observe that
%   \begin{align*}
%     I-(I+\Delta)^{-1}
%     &= \Delta(I+\Delta)^{-1} \\
%     &= \hat{\Sigma}^{-1/2}(\Sigma_{B \cap R} - \hat{\Sigma}_{G'})\hat{\Sigma}^{-1/2}
%       (I + \hat{\Sigma}^{-1/2}(\Sigma_{B \cap R} - \hat{\Sigma}_{G'})\hat{\Sigma}^{-1/2})^{-1} \\
%     &= \hat{\Sigma}^{-1/2}(\Sigma_{B \cap R} - \hat{\Sigma}_{G'})
%     (\hat{\Sigma} + \Sigma_{B \cap R} - \hat{\Sigma}_{G'})^{-1}\hat{\Sigma}^{1/2}.
%   \end{align*}
%   Notice that $\tr(|\cdot|)$ is the nuclear norm of a matrix, and so triangle
%   inequality implies that
%   \begin{align*}
%     \tr(|I-(I+\Delta)^{-1}|)
%     &\leq \tr(|\hat{\Sigma}^{-1/2}\Sigma_{B \cap R}
%       (\hat{\Sigma} + \Sigma_{B \cap R} - \hat{\Sigma}_{G'})^{-1}\hat{\Sigma}^{1/2}|) \\
%     &\qquad + \tr(|\hat{\Sigma}^{-1/2}\Sigma_{G'}
%         (\hat{\Sigma} + \Sigma_{B \cap R} - \hat{\Sigma}_{G'})^{-1}\hat{\Sigma}^{1/2}|). \\
%   \end{align*}
%   Then, we have that
%   Expanding out $\hat{\Sigma}_{G'}$, we have
%   \begin{align*}
%     \tr(\hat{\Sigma}^{-1/2}\hat{\Sigma}_{G'}\hat{\Sigma}^{-1/2})
%      & = \frac{1}{n}\sum_{k \in G'} x_k^T \hat{\Sigma}^{-1} x_k
%     \leq \ti{O}(d|G'|/n)
%     = \ti{O}(\eps d).
%   \end{align*}
%   Similarly
%   \begin{align*}
%     \tr(\hat{\Sigma}^{-1/2}\Sigma_{B \cap R}\hat{\Sigma}^{-1/2})
%     & = \frac{1}{n}\sum_{k \in B \cap R} x_k^T \hat{\Sigma}^{-1} x_k
%     \leq \ti{O}(d|B \cap R|/n)
%     = \ti{O}(\eps d)
%   \end{align*}


%   which thus implies $\P(y_i^T |\Delta| y_i \gtrsim 1/\eps) = \ti{O}(\eps^2 d)$
%   and hence $|S| = \ti{O}(\eps^2 d) n$.

%   This proves the desired result.
% \end{proof}

==> sections/results.tex <==
\section{Results}
